Spatial Distribution Patterns of Clownfish in Recirculating Aquaculture Systems

Successful aquaculture systems can reduce the pressure and help secure the most diverse and productive Red Sea coral reef ecosystem to maintain a healthy and functional ecosystem within a sustainable blue economy. Interestingly, recirculating aquaculture systems are currently emerging in fish farm production practices. On the other hand, monitoring and detecting fish behaviors provide essential information on fish welfare and contribute to an intelligent production in global aquaculture. This work proposes an efficient approach to analyze the spatial distribution status and motion patterns of juvenile clownfish \textit{(Amphiprion bicinctus)} maintained in aquaria at three stocking densities (1, 5, and 10 individuals/aquarium). The estimated displacement is crucial in assessing the dispersion and velocity to express the clownfish's spatial distribution and movement behavior in a recirculating aquaculture system. Indeed, we aim to compute the velocity, magnitude, and turning angle using an optical flow method to assist aquaculturists in efficiently monitoring and identifying fish behavior. We test the system design on a database containing two days of video streams of juvenile clownfish maintained in aquaria. The proposed displacement estimation reveals good performance in measuring clownfish's motion and dispersion characteristics leading to assessing the potential signs of stress behaviors. We demonstrate the effectiveness of the proposed technique for quantifying variation in clownfish activity levels between recordings taken in the morning and afternoon at different stocking densities. It provides practical baseline support for online predicting and monitoring feeding behavior in ornamental fish aquaculture.

==> README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> arxiv-style-master Spatial Patterns of Clownfish v3/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> arxiv-style-master Spatial Patterns of Clownfish v3/setup-IEEEtrans.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%      setup pour articles     %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%% reglages des flottants %%%%%%%%%%%%%%%%%%%%
\renewcommand{\floatpagefraction}{.95} % les flottants peuvent occuper
% 95% de la page
\renewcommand{\textfraction}{.1} % le texte peut n'occuper que 10% de
% la page
\renewcommand{\dblfloatpagefraction}{.99} % les flottants en twocolumn
% peuvent occuper 90% de la page
\renewcommand{\dbltopfraction}{0.90} % 90% du top peut etre occup� par
% les flottants en twocolumn
\renewcommand{\dblfloatsep}{0pt} % espace entre flottants et d�but/fin
% de la page en twocolumn
\renewcommand{\dbltextfloatsep}{0pt} % espace entre flottants du d�but/fin
% de la page et texte en twocolumn
\renewcommand{\intextsep}{0pt} % espace vertical entre flottants et
% texte en twocolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% modification de l'interligne (80% de l'original)
% \renewcommand{\baselinestretch}{.8}

% To adjust the position of the text on the page
% (for our specific printer) with the commands
%            \addtolength{\oddsidemargin}{Xmm} % right Xmm
%           \addtolength{\topmargin}{Ymm}     % down Ymm

% \addtolength{\topmargin}{10mm} %rajoute 1 cm en haut de la page

% \setlength{\labelsep}{1pt}
% \setlength{\itemsep}{0pt}

% espaces dans les tableaux
\renewcommand{\arraystretch}{1.3} % diminue hauteur des lignes dans tableaux
% \setlength{\arraycolsep}{1pt}
\setlength{\arraycolsep}{5pt} % espace entre les colonnes (array et matrix)
\setlength{\tabcolsep}{1pt}
% \addtolength{\doublerulesep}{-1pt} % espace entre double trait
% \addtolength{\extratabsurround}{-2pt}

%% listes compactes avec mdwlist
%\makecompactlist{enumerateb}{enumerate}
%\makecompactlist{itemizeb}{itemize}
%\makecompactlist{descriptionb}{description}

\allowdisplaybreaks % Autorise la coupure de fin de page

% red�finition des tailles exposants/indices maths %%change HS 15-05-2001
% \DeclareMathSizes{12}{12}{7}{5}
% \DeclareMathSizes{11}{11}{7}{5}
% \DeclareMathSizes{10}{9}{6}{4}

% Spaces before and after environment EQ
\setlength{\abovedisplayskip}{1 mm}
\setlength{\belowdisplayskip}{1 mm}
\setlength{\abovedisplayshortskip}{1 mm}
\setlength{\belowdisplayshortskip}{1 mm}

% Affiche des numeros jusq'au paragraph
\setcounter{secnumdepth}{4}
% profondeur de la toc
\setcounter{tocdepth}{4} % jusqu'a sous-section
% profondeur de la lof
% \setcounter{lofdepth}{3} % jusqu'a caption "x.a", "x.b"

% rajoute de la hauteur de page
% \addtolength{\textheight}{0.2in}
% \addtolength{\headsep}{-2mm}

% permet une num�rotation des �quations en rapport avec la section
% \numberwithin{equation}{section}
% \numberwithin{newenvironment}{section}

% permet une sous-num�rotation en lettres dans subequations et
% subeqnarray
% \def\theequation{\alph{equation}}
% \def\thesubequation{\theequation\alph{subequation}}
% \renewcommand{\theequation}{\theparentequation\alph{equation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Attention -- ancienne version --
% permet une sous-num�rotation en lettres dans subequations
% � inserer � l'int�rieur de l'environnement subequations
% \renewcommand{\thesubequation}{\theequation\alph{subequation}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%% Red�finition des sections
% \def\thesection {\arabic{section}.}
% \def\thesubsection {\thesection\arabic{subsection}.}
% \def\thesubsubsection {\thesubsection\arabic{subsubsection}.}
% \def\theparagraph {\thesubsubsection\arabic{paragraph}.}
% \def\thesubparagraph {\theparagraph\arabic{subparagraph}.}

% permet une �num�ration (i),(ii),(iii)
% \def\labelenumi{(\bf\theenumi)}     \def\theenumi{\roman{enumi}}
% \def\labelenumii{\bf\theenumii}  \def\theenumii{$\scriptstyle\bullet$}
% \def\labelenumiii{\theenumiii.} \def\theenumiii{\arabic{enumiii}}
% \def\labelenumiv{\theenumiv.}   \def\theenumiv{\alph{enumiv}}
% \def\p@enumii{\theenumi}
% \def\p@enumiii{\theenumi(\theenumii)}
% \def\p@enumiv{\p@enumiii\theenumiii}

% D�finition de la date du jour en Fran�ais
\def\aujour{\number\day \space \ifcase\month\or
janvier\or f�vrier\or mars\or avril\or mai\or
juin\or juillet\or ao�t\or septembre\or octobre\or
novembre\or d�cembre\fi \space \number\year}

% diff�rents espaces verticaux sans indentations apr�s
\newcommand{\petesp}{{\smallskip \noindent}}
\newcommand{\moyesp}{{\medskip \noindent}}
\newcommand{\graesp}{{\bigskip \noindent}}
\newcommand{\ggraesp}{{\bigskip \bigskip \noindent}}

\newcommand{\nid}{{\noindent}}

% en gras
\def\bA{{\bf A}}
\def\bB{{\bf B}}
\def\bC{{\bf C}}
\def\bD{{\bf D}}
\def\bBu{{{\bf B}_u}}
\def\bBw{{{\bf B}_w}}
\def\bCy{{{\bf C}_y}}
\def\bDyu{{{\bf D}_{yu}}}
\def\bDyw{{{\bf D}_{yw}}}
\def\bCz{{{\bf C}_z}}
\def\bDzu{{{\bf D}_{zu}}}
\def\bDzw{{{\bf D}_{zw}}}
\def\bE{{\bf E}}
\def\bF{{\bf F}}
\def\bG{{\bf G}}
\def\bH{{\bf H}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bK{{\bf K}}
\def\bL{{\bf L}}
\def\bM{{\bf M}}
\def\bN{{\bf N}}
\def\bO{{\bf O}}
\def\bP{{\bf P}}
\def\bQ{{\bf Q}}
\def\bR{{\bf R}}
\def\bS{{\bf S}}
\def\bT{{\bf T}}
\def\bU{{\bf U}}
\def\bV{{\bf V}}
\def\bW{{\bf W}}
\def\bX{{\bf X}}
\def\bY{{\bf Y}}
\def\bZ{{\bf Z}}

% en calligraphi�
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

\def\cIr{{\cal I}(r)}
\def\cSr{{\cal S}(r)}
\def\cBr{{\cal B}(r)}
\def\cDr{{\cal D}(r)}
\def\cGr{{\cal G}(r)}
\def\cFl{{\cal F}_{l}}
\def\cFu{{\cal F}_{u}}
\def\cEP{\mbox{${\cal E}_P$}}
\def\cEQinv{\mbox{${\cal E}_{Q^{-1}}$}}

% widetilde
\def\tA{{\widetilde{A}}}
\def\tB{{\widetilde{B}}}
\def\tC{{\widetilde{C}}}
\def\tD{{\widetilde{D}}}
\def\tE{{\widetilde{E}}}
\def\tF{{\widetilde{F}}}
\def\tG{{\widetilde{G}}}
\def\tH{{\widetilde{H}}}
\def\tI{{\widetilde{I}}}
\def\tJ{{\widetilde{J}}}
\def\tK{{\widetilde{K}}}
\def\tL{{\widetilde{L}}}
\def\tM{{\widetilde{M}}}
\def\tN{{\widetilde{N}}}
\def\tO{{\widetilde{O}}}
\def\tP{{\widetilde{P}}}
\def\tQ{{\widetilde{Q}}}
\def\tR{{\widetilde{R}}}
\def\tS{{\widetilde{S}}}
\def\tT{{\widetilde{T}}}
\def\tU{{\widetilde{U}}}
\def\tV{{\widetilde{V}}}
\def\tW{{\widetilde{W}}}
\def\tX{{\widetilde{X}}}
\def\tY{{\widetilde{Y}}}
\def\tZ{{\widetilde{Z}}}
\def\tek{{\widetilde{e}}_k}
\def\tr{{\widetilde{r}}}
\def\tx{{\widetilde{x}}}

% overline
\def\oA{{\overline{A}}}
\def\oB{{\overline{B}}}
\def\oC{{\overline{C}}}
\def\oD{{\overline{D}}}
\def\oE{{\overline{E}}}
\def\oF{{\overline{F}}}
\def\oG{{\overline{G}}}
\def\oH{{\overline{H}}}
\def\oI{{\overline{I}}}
\def\oJ{{\overline{J}}}
\def\oK{{\overline{K}}}
\def\oL{{\overline{L}}}
\def\oM{{\overline{M}}}
\def\oN{{\overline{N}}}
\def\oO{{\overline{O}}}
\def\oP{{\overline{P}}}
\def\oQ{{\overline{Q}}}
\def\oR{{\overline{R}}}
\def\oS{{\overline{S}}}
\def\oT{{\overline{T}}}
\def\oU{{\overline{U}}}
\def\oV{{\overline{V}}}
\def\oW{{\overline{W}}}
\def\oX{{\overline{X}}}
\def\oY{{\overline{Y}}}
\def\oZ{{\overline{Z}}}
\def\ova{{\overline{a}}}
\def\ovb{{\overline{b}}}
\def\ovx{{\overline{x}}}
\def\ovg{{\overline{g}}}
\def\ovr{{\overline{r}}}

% widehat
\def\hA{{\widehat{A}}}
\def\hB{{\widehat{B}}}
\def\hC{{\widehat{C}}}
\def\hD{{\widehat{D}}}
\def\hE{{\widehat{E}}}
\def\hF{{\widehat{F}}}
\def\hG{{\widehat{G}}}
\def\hH{{\widehat{H}}}
\def\hI{{\widehat{I}}}
\def\hJ{{\widehat{J}}}
\def\hK{{\widehat{K}}}
\def\hL{{\widehat{L}}}
\def\hM{{\widehat{M}}}
\def\hN{{\widehat{N}}}
\def\hO{{\widehat{O}}}
\def\hP{{\widehat{P}}}
\def\hQ{{\widehat{Q}}}
\def\hR{{\widehat{R}}}
\def\hS{{\widehat{S}}}
\def\hT{{\widehat{T}}}
\def\hU{{\widehat{U}}}
\def\hV{{\widehat{V}}}
\def\hW{{\widehat{W}}}
\def\hX{{\widehat{X}}}
\def\hY{{\widehat{Y}}}
\def\hZ{{\widehat{Z}}}
\def\whx{{\widehat{x}}} % MZ
\def\whw{{\widehat{w}}} % MZ
\def\whz{{\widehat{z}}} % MZ

% orthogonaux
\def\orthU{{U_{\rm orth}}}
\def\orthV{{V_{\rm orth}}}
\def\pU{{U_{\perp}}}
\def\pV{{V_{\perp}}}
\def\torthU{{\tilde{U}_{\rm orth}}}
\def\torthV{{\tilde{V}_{\rm orth}}}

% math environnements
% \def\BA[{\left[\begin{array}} % a revoir
% \def\BEAS{\begin{eqnarray*}} % a revoir
% \def\BEA{\begin{eqnarray}} % a revoir
% \def\BEQ{\begin{equation}} % a revoir
% \def\Co{{\mathop {\bf Co}}} % a revoir
% \def\EA]{\end{array}\right]} % a revoir
% \def\EEAS{\end{eqnarray*}} % a revoir
% \def\EEA{\end{eqnarray}} % a revoir
% \def\EEQ{\end{equation}} % a revoir
% \newcommand{\EEL}[1]{\label{#1}\end{equation}} % a revoir

% New environments thms, etc
% \theoremstyle{plain} % avec num�rotation relative selon les sections
% \newtheorem{thm}{Theorem}[section]
% \newtheorem{cor}[thm]{Corollary}
% \newtheorem{prop}[thm]{Proposition}
% \newtheorem{lemma}[thm]{Lemma}
% \newtheorem{proper}[thm]{Property}
%\newtheorem{defi}[thm]{Definition}
% \newtheorem{prob}[thm]%{Problem}

% % \theoremstyle{definition}
% % \newtheorem{defi}{Definition}[section]

% \theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{ass}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{col}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{defi}{Definition}
%\newtheorem{proof}{Proof}
% \theoremstyle{algo}
% \newtheorem{algo}[thm]{Algorithm}%{Algorithme}

% \newass{ass}{Assumption}
%
% % avec ou sans num�rotation selon les section et non relative
% \theoremstyle{plain}
% \newtheorem{defi}{Definition}%{D�finition}%[section]
% \newtheorem{lemma}{Lemma}%{Lemme}%[section]
% \newtheorem{cor}{Corollary}%{Corollaire}%[section]
% \newtheorem{thm}{Theorem}%{Th�or�me}%[section]
% \newtheorem{prop}{Proposition}%{Proposition}%[section]
%  % \newtheorem{ass}{Assumption}%{Hypoth�se}%[section]
% \newtheorem{proper}{Property}%{Propri�t�}%[section]
% \newtheorem{prob}{Problem}%{Probl�me}%[section]

%\newtheorem{thm}{Theorem}%{Th\'eor\`eme}%{Th�or�me}%[section]
%% \newtheorem{defi}{Definition}%{D�finition}%[section]
%\newtheorem{lem}{Lemma}%{Lemme}%[section]
%\newtheorem{col}{Corollary}%{Corollaire}%{Corollary}%{Corollaire}%[section]
%\newtheorem{prop}{Proposition}%{Proposition}%[section]
%% \newtheorem{ass}{Assumption}%{Hypoth�se}%[section]
%\newtheorem{proper}{Property}%{Propri�t�}%[section]
%% \newtheorem{prob}{Problem}%{Probl�me}%[section]
%% \newtheorem*{prob*}{Problem} % sans numeotation (amsthm)
%%\newtheorem{proo}{Proof}%{Probl�me}%[section]
%% \theoremstyle{remark} % corps en caract�res droit
%% \newtheorem{remark}{Remark}%{Remarque}%[section]

%\theoremstyle{definition}
%\newtheorem{defi}{Definition} %{D�finition}%[section]
%\newtheorem{prob}{Problem} %{Probl�me}%[section]
%\newtheorem*{prob*}{Problem} % sans numerotation (amsthm)
%\newtheorem{remark}{Remarque}%{Remark} %{Remarque}%[section]
%\newtheorem*{remark*}{Remark} % sans numerotation (amsthm)
%\newtheorem{ass}{Assumption}%{Hypoth\`ese}%{Assumption}%{Hypoth�se}%[section]
%%\newtheorem{proo}{Proof}
%% \theoremstyle{algo}
%\newtheorem{algo}{Algorithm}%{Algorithme}%[chapter]

\newcommand{\ethm}{\ding{110}}%charact�re fin_de_th�or�me
\newcommand{\elem}{$\square$}%charact�re fin_de_lemme
\newcommand{\edefini}{\ding{117}}%charact�re fin_de_d�finition
\newcommand{\eass}{\ding{114}}%charact�re fin_d'assumption
\newcommand{\ermk}{\ding{113}}%charact�re fin_de_remarque
\newcommand{\eprop}{\ding{109}}%charact�re fin_de_proposition

% \renewcommand{\qedsymbol}{\ding{111}}
%\renewcommand{\qedsymbol}{$\large\bullet$}

\newcommand{\units}[2]{#1\textrm{\thinspace \thinspace #2}} %unit�s de mesure

% d�finitions des ensembles Math�matiques
%%% Cr�ations EM
\def\C{{\setbox0=\hbox{$\displaystyle{\rm C}$}
        \hbox{\hbox to0pt{\kern 0.4\wd0\vrule height 0.95\ht0\hss}\box0}}}
        % ensemble des Complexes --> OK
\def\Q{{\setbox0=\hbox{$\displaystyle{\rm Q}$}%
    \hbox{\raise 0.2\ht0\hbox to0pt{\kern 0.4\wd0\vrule height
    0.85\ht0\hss}\box0}}} % ensemble des Rationnels --> � revoir
\def\R{\mathop{\rm I\mkern -3.5mu R}} % ensemble des R�els --> OK
%\def\Z{\mathop{\rm I\mkern -3.5mu Z}} % ensemble des R�els --> OK
\def\N{\mathop{\rm I\mkern -3.5mu N}} % ensemble des Entiers --> OK
\def\Cij{{\C}^{i\times j}}
\def\Cn{{\C}^n}
\def\Rij{{\R}^{i\times j}}
\def\Rj{{\R}^j}
\def\Rji{{\R}^{j\times i}}
\def\Rjrmi{{\R}^{(j+r)\times (m+i)}}
\def\Rjrnur{{\R}^{(j+r)\times (n_{1}+r)}}
\def\Rk{{\R}^k}
\def\Rki{{\R}^{k_{i}}}
\def\Rkk{{\R}^{k\times k}}
\def\Rokok{{\R}^{\overline{k}\times \overline{k}}}
\def\Rkiki{{\R}^{k_{i}\times k_{i}}}
\def\Rkl{{\R}^{(k+\ell)}}
\def\Rklkl{{\R}^{(k+\ell)\times (k+\ell)}}
\def\Rksiksi{{\R}^{k_{s+i}\times k_{s+i}}}
\def\Rell{{\R}^{\ell}}
\def\Rm{{\R}^m}
\def\Rmone{{\R}^{m_{1}}}
\def\Rmtwo{{\R}^{m_{2}}}
\def\Rmoneone{{\R}^{m_{1}\times m_{1}}}
\def\Rmtwotwo{{\R}^{m_{2}\times m_{2}}}
\def\Rmn{{\R}^{m\times n}}
\def\Rmq{{\R}^{m\times q}}
\def\Rn{{\R}^n}
\def\Rden{{\R}^{2n}}
\def\Rnone{{\R}^{n_{1}}}
\def\Rntwo{{\R}^{n_{2}}}
\def\Rnk{{\R}^{n+k}}
\def\Rnm{{\R}^{n\times m}}
\def\Rnmnm{{\R}^{(n+m)\times (n+m)}}
\def\Rnurmi{{\R}^{(n_{1}+r)\times (m+i)}}
\def\Rnn{{\R}^{n\times n}}
\def\RNN{{\R}^{N\times N}}
\def\Rnnu{{\R}^{n\times n_{u}}}
\def\Rnunu{{\R}^{n_{1}\times n_{1}}}
\def\Rnurnur{{\R}^{(n_{1}+r)\times (n_{1}+r)}}
\def\Rnnw{{\R}^{n\times n_{w}}}
\def\Rnny{{\R}^{n\times n_{y}}}
\def\Rnp{{\R}^{n\times p}}
\def\Rnpp{{\R}^{n-p}}
\def\Rnpn{{\R}^{(n-p)\times n}}
\def\Rnurdp{{\R}^{(n_{1}+r)\times 2p}}
\def\Rnrnr{{\R}^{(n+r)\times (n+r)}}
\def\Rnq{{\R}^{n\times q}}
\def\Rnr{{\R}^{n\times r}}
\def\Rp{{\R}^p}
\def\Rpone{{\R}^{p_{1}}}
\def\Rptwo{{\R}^{p_{2}}}
\def\Rpn{{\R}^{p\times n}}
\def\Rpq{{\R}^{p\times q}}
\def\Rdpmi{{\R}^{2p\times (m+i)}}
\def\Rdpnur{{\R}^{2p\times (n_{1}+r)}}
\def\Rponeone{{\R}^{p_{1}\times p_{1}}}
\def\Rptwotwo{{\R}^{p_{2}\times p_{2}}}
\def\Rq{{\R}^q}
\def\Rqone{{\R}^{q_{1}}}
\def\Rqtwo{{\R}^{q_{2}}}
\def\Rqq{{\R}^{q\times q}}
\def\Rqoneone{{\R}^{q_{1}\times q_{1}}}
\def\Rqtwotwo{{\R}^{q_{2}\times q_{2}}}
\def\Rr{{\R}^r}
\def\Rrone{{\R}^{r_{1}}}
\def\Rrtwo{{\R}^{r_{2}}}
\def\Rrn{{\R}^{r\times n}}
\def\Rrp{{\R}^{r\times p}}
\def\Rrdp{{\R}^{r\times 2p}}
\def\Rrr{{\R}^{r\times r}}
\def\Rs{{\R}^s}
\def\Rv{{\R}^v}
\def\Rvone{{\R}^{v_{1}}}
\def\Rvtwo{{\R}^{v_{2}}}
\def\Rvv{{\R}^{v\times v}}
%% versions newsgroup "fr.comp.text.tex"
\def \ensN {\mbox{I\hspace{-.15em}N}}
\def \ensR {\mbox{I\hspace{-.15em}R}}
\def \ensZ {\mbox{Z\hspace{-.32em}Z}}
\def \ensC {\mbox{l\hspace{-.47em}C}}
\def \ensQ {\mbox{l\hspace{-.47em}Q}}
% autre d�finition de Z et de N
% \newcommand{\Z}{$\Bbb Z$}                 % D�finition du Z math�matique
% \newcommand{\N}{{\it I\!\!N}}             % D�finition du N math�matique
% \newcommand{\ZZ}{\mathbb{Z}}              % D�finition du Z math�matique
% \newcommand{\NN}{\mathbb{N}}              % D�finition du N math�matique

% math symbols and operators
\def\Expect{\mathop{\bf E}} % esp�rance

% \def\cHi{\mathop{{\mathcal{H}}_{\infty}} % Hinf calligraphi� (norme)
% \def\cH2{\mathop{{\mathcal{H}}_2} % H2 calligraphi� (norme)
\def\cHi{{\cal H}_{\infty}} % Hinf calligraphi� (norme)
\def\cH2{{\cal H}_2} % H2 calligraphi� (norme)
\def\cU{{\cal U}}

\def\cLi{\mathop{\mathcal L}_{\infty}} % Linf
\def\cLone{\mathop{\mathcal L}_{1}} % L1
\def\cL2{\mathop{\mathcal L}_{2}} % espace carr�-int�grable
%en continu
\def\cHinfc{{\cal H}_{\infty}^c} % espace Banach pour continu
\def\cHtwoc{{\cal H}_2^c} % espace Hilbert pour continu
%en discret
\def\cHinfd{{\cal H}_{\infty}^d} % espace Banach pour discret
\def\cHtwod{{\cal H}_2^d} % espace Hilbert pour discret

\def\cRHi{\mathop{\cal R \cal H}_\infty} % RHinf calligraphi� (norme)
\def\cRH2{\mathop{\cal R \cal H}_2} % RH2 calligraphi� (norme)
\def\cRLi{\mathop{\cal R \cal L}_{\infty}} % RLinf
\def\cRLone{\mathop{\cal R \cal L}_{1}} % RL1
\def\cRL2{\mathop{\cal R \cal L}_{2}} % espace carr�-int�grable

\def\Ltwo{{\bf L}_2}

% \def\Reel{\mbox{\bf Re}}
% \def\Im{\mbox{\bf Im}}
%
% \def\log{\mbox{\bf log}}
% \def\det{\mbox{\bf det}}
% \def\rank{\mbox{\bf rank}}
% \def\tra{\mathop{\bf tr}}
% \def\diag{\mbox{\bf diag}}
% \def\bdiag{\mbox{\bf bdiag}}
% \def\herm{\mbox{\bf herm}}
% \def\ker{\mbox{\bf ker}}
% \def\image{\mbox{\bf span}}
% \def\cond{\mbox{\bf cond}}
% \def\min{\mbox{\bf min}}
% \def\max{\mbox{\bf max}}
% \def\dim{\mbox{\bf dim}}
% \def\deg{\mbox{\bf deg}}
% \def\exp{\mbox{\bf exp}}
% \def\lim{\mbox{\bf lim}}

\def\Prob{\mathop{\bf Prob}}

\def\sat{\mbox{\bf sat}}

% \def\Reel{\mbox{Re}}
% \def\Im{\mbox{Im}}
%
% \def\det{\mbox{det}}
% \def\rank{\mbox{rank}}
% \def\tra{\mathop{tr}}
% \def\diag{\mbox{diag}}
% \def\bdiag{\mbox{bdiag}}
% \def\herm{\mbox{herm}}
% \def\ker{\mbox{ker}}
% \def\image{\mbox{span}}
% \def\cond{\mbox{cond}}
% \def\min{\mbox{min}}
% \def\max{\mbox{max}}
% \def\dim{\mbox{dim}}
% \def\deg{\mbox{deg}}
% \def\exp{\mbox{exp}}
% \def\lim{\mbox{lim}}
\DeclareMathOperator*{\bdiag}{bdiag}
\DeclareMathOperator*{\dcond}{cond}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\esp}{Esp}
\DeclareMathOperator*{\herm}{herm}
\DeclareMathOperator*{\im}{Im}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator*{\re}{Re}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\atan}{atan}
% \DeclareMathOperator*{\span}{span}
\DeclareMathOperator*{\trace}{tr}
\DeclareMathOperator*{\vect}{vect}
\DeclareMathOperator*{\vectb}{vectb}
\def\vectbc{\mbox{vectb}_{\textrm{c}}}
\def\vectbr{\mbox{vectb}_{\textrm{r}}}
\DeclareMathOperator*{\with}{with}
\DeclareMathOperator*{\der}{d}
\DeclareMathOperator*{\Sym}{Sym}
\DeclareMathOperator*{\spec}{spec}
\DeclareMathOperator*{\eig}{eig}

% fonction de normes, abs, norme Hinf, norme H2, norm Linf et norme L2
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\norminf}[1]{{\left\|{#1}\right\|}_{\infty}}
\newcommand{\normtwo}[1]{{\left\|{#1}\right\|}_{2}}
\newcommand{\normLinf}[1]{{\left\|{#1}\right\|}_{{\cal L}_{\infty}}}
\newcommand{\normLtwo}[1]{{\left\|{#1}\right\|}_{{\cal L}_{2}}}

% double overline
\newcommand{\bbar}[1]{\overline{\overline{#1}}}

% regular height vertical bar
\def\setmid{\, \mid \,}
% scalable vertical bar (must be paired with \right.)
\def\leftsetmid{ \; \left| \; }
% scalable vertical bar (must be paired with \left.)
\def\rightsetmid{ \; \right| \; }

%\renewcommand{\QED}{\textbullet}
%\def\QED{~~\rule[-1pt]{8pt}{8pt}}\def\qed{\QED}
\def\qedsymbol{\textbullet}
%\renewcommand{\proofname}{Proof}
%\def\TheWordProof{D�monstration\enskip}

\def\SAT{\mbox{SAT}}
\def\SD{\mbox{SD}}

%\def\approxeq{\approx}
%\def\approxleq{\mathrel{\smash{\makebox[0pt][l]{\raisebox{-3.4pt}
%{\small$\sim$}}}{\raisebox{1.1pt}{$<$}}}}
\def\argmin{\mathop{\rm argmin}}
\def\eqbydef{\mathrel{\stackrel{\Delta}{=}}}
\def\infeqyn{\mathrel{\stackrel{{\large ?}}{\leqslant}}}
\def\supeqyn{\mathrel{\stackrel{{\large ?}}{\geqslant}}}

\def\mini{\mathop{\min}} % � utiliser avec par exemple
% "\underset{X\in\Phi}{\mini}\; V(X)"
\def\maxi{\mathop{\max}} % � utiliser avec par exemple
% "\underset{X\in\Phi}{\maxi}\; V(X)"
\def\limi{\mathop{\lim}}

%\newcommand{\mina}[1]{\mathrel{\stackrel{\min}{#1}}}
%\newcommand{\maxa}[1]{\mathrel{\stackrel{\max}{#1}}}
% � utiliser avec \mina{xxx} ou bien maxa{xxx}

%\newcommand{\sigmaM}{{\ensuremath{\sigma_{\max}}}}
\newcommand{\sigmaM}{\ensuremath{\overline{\sigma}}}
%\newcommand{\sigmam}{\ensuremath{\sigma_{\min}}}
\newcommand{\sigmam}{\ensuremath{\underline{\sigma}}}
\newcommand{\lambdaM}{\ensuremath{\lambda_{\rm max}}}
\newcommand{\lambdam}{\ensuremath{\lambda_{\rm min}}}
\def\argmax{{\mbox{argmax}}}
\def\lambdaopt{\lambda^{\rm opt}}

\def\xst{{x^{*}}}
\def\xopt{{x^{\rm opt}}}
\def\lambdak{{\lambda^{(k)}}}
\def\lambdakp{{\lambda^{(k+1)}}}

\def\Aaug{A_{\rm aug}}
\def\Baug{B_{\rm aug}}
\def\Bpaug{B_{{\rm aug},\, p}}
\def\Bwaug{B_{{\rm aug},\, w}}
\def\Cqaug{C_{{\rm aug},\,q}}
\def\Dqpaug{D_{{\rm aug},\, qp}}
\def\Czaug{C_{{\rm aug},\,z}}
\def\xaug{x_{\rm aug}}
\def\Paug{P_{\rm aug}}

% text abbrevs
\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\nd}[1]{${#1}^{\textrm{nd}}$}
\newcommand{\st}[1]{${#1}^{\textrm{st}}$}
\newcommand{\thh}[1]{${#1}^{\textrm{th}}$}
\newcommand{\rd}[1]{${#1}^{\textrm{rd}}$}
\newcommand{\eme}[1]{${#1}^{\textrm{\`eme}}$}
\newcommand{\ere}[1]{${#1}^{\textrm{\`ere}}$}
\newcommand{\er}[1]{${#1}^{\textrm{er}}$}
\newcommand{\eal}{{\it et al.\ }}
%\newcommand{\eqref}[1]{\mbox{(\ref{#1})}}
%\newcommand{\frgui}[1]{``{#1}''} % french guillemets --> OK
\newcommand{\frgui}[1]{`{#1}'}
\newcommand{\frguib}[1]{``{#1}''}

\newcommand{\dis}[1]{\displaystyle{#1}}
% espace top et bottom dans ligne de array% a utiliser avec \Ts et \Bs
\newcommand\setTBstruts{\def\Ts{\rule{0pt}{2.6ex}}%
                        \def\Bs{\rule[-1.2ex]{0pt}{0pt}}}

\newcommand{\XXX}[1]{\marginpar{\raggedright \footnotesize #1}}

% nom du label pour figures : Fig.
% \renewcommand\figurename{fig.}
%
% \renewcommand\tablename{\textbf{tab.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sfrac : ecrire proprement a/b
\makeatletter
\DeclareRobustCommand\sfrac[1]{\@ifnextchar/{\@sfrac{#1}}
                                            {\@sfrac{#1}/}}
\def\@sfrac#1/#2{\leavevmode\kern.1em\raise.5ex
         \hbox{$\m@th\fontsize\sf@size\z@
                           \selectfont#1$}\kern-.1em
         /\kern-.15em\lower.25ex
          \hbox{$\m@th\fontsize\sf@size\z@
                            \selectfont#2$}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% plotting command
\newcommand{\mplot}[4]{
    \begin{figure}[ftb]
    \begin{center}
    \unitlength 0.30 truein
    \begin{picture}(10,10)(6,6.5)
    \special{psfile = #1.ps hscale=70 vscale=70}
    \put(10,6.4){#3}
    \put(.5,13){#4}
    \end{picture}
    \caption{#2}
    \label{fig:#1}
    \end{center}
    \end{figure}
}

\newcommand{\mplotm}[4]{
    \begin{figure}[ftb]
    \begin{center}
    \unitlength 0.15 truein
    \begin{picture}(10,12)(6,6.5)
    \special{psfile = #1.ps hscale=35 vscale=35}
    \put(10,6.1){{\small #3}}
    \put(.5,13){{\small #4}}
    \end{picture}
    \caption{#2}
    \label{fig:#1}
    \end{center}
    \end{figure}
}

\newcommand{\mplotlr}[7]{
\begin{figure}[ftb]
     \unitlength 0.15 truein
     \begin{picture}(10,12)(6,6.5)
           \put(5,0){\special{psfile = #1.ps hscale=35 vscale=35}}
           \put(15,6.1){{\small #3}}
       \put(5.5,13){{\small #4}}
           \put(25,0){\special{psfile = #5.ps hscale=35 vscale=35}}
           \put(35,6.1){{\small #6}}
       \put(25.5,13){{\small #7}}
     \end{picture}
\caption{#2}
\label{fig:#1}
\end{figure}
}

